GRIM: A General, Real-Time Deep Learning Inference Framework for Mobile Devices based on Fine-Grained Structured Weight Sparsity

It is appealing but challenging to achieve real-time deep neural network (DNN) inference on mobile devices because even the powerful modern mobile devices are considered as ``resource-constrained'' when executing large-scale DNNs. It necessitates the sparse model inference via weight pruning, i.e., DNN weight sparsity, and it is desirable to design a new DNN weight sparsity scheme that can facilitate real-time inference on mobile devices while preserving a high sparse model accuracy. This paper designs a novel mobile inference acceleration framework GRIM that is General to both convolutional neural networks (CNNs) and recurrent neural networks (RNNs) and that achieves Real-time execution and high accuracy, leveraging fine-grained structured sparse model Inference and compiler optimizations for Mobiles. We start by proposing a new fine-grained structured sparsity scheme through the Block-based Column-Row (BCR) pruning. Based on this new fine-grained structured sparsity, our GRIM framework consists of two parts: (a) the compiler optimization and code generation for real-time mobile inference; and (b) the BCR pruning optimizations for determining pruning hyperparameters and performing weight pruning. We compare GRIM with Alibaba MNN, TVM, TensorFlow-Lite, a sparse implementation based on CSR, PatDNN, and ESE (a representative FPGA inference acceleration framework for RNNs), and achieve up to 14.08x speedup.

==> Texs/drafts.tex <==


% \begin{itemize}
%     \item How to make IR generality ?
%     \item How to solve tiny and skinny GEMM?
%     \item How to reduce Im2col/GEMM overhead?
%     \item How to store data for block-based CONV?
%     \item How to decide block count/size and pruning rate?
%     \item How to distinguish TVM/Halide/Taco and ours?
%     \item How to avoid copy data multi times when we divide weights to $k \times h$?
% \end{itemize}



% Why not CONV directly or Why choose GEMM?
% \begin{itemize}
%     \item Because block-based pruning has uncertainty, different filters in different block has different kernel styles.
% \end{itemize}

% Assumption:
% \begin{itemize}
%     \item Graph partition - Static Memory management
% \end{itemize}


